DNS of the kappa-mechanism

We present a purely-radiative hydrodynamic model of the kappa-mechanism that sustains radial oscillations in Cepheid variables. We determine the physical conditions favourable for the kappa-mechanism to occur by the means of a configurable hollow in the radiative conductivity profile. By starting from these most favourable conditions, we complete nonlinear direct numerical simulations (DNS) and compare them with the results given by a linear-stability analysis of radial modes. We find that well-defined instability strips are generated by changing the location and shape of the conductivity hollow. For a given position in the layer, the hollow amplitude and width stand out as the key parameters governing the appearance of unstable modes driven by the kappa-mechanism. The DNS confirm both the growth rates and structures of the linearly-unstable modes. The nonlinear saturation that arises is produced by intricate couplings between the excited fundamental mode and higher damped overtones. These couplings are measured by projecting the DNS fields onto an acoustic subspace built from regular and adjoint eigenvectors and a 2:1 resonance is found to be responsible for the saturation of the kappa-mechanism instability.

==> Makefile <==
# $Id: Makefile,v 1.1.1.1 2008/09/10 13:47:08 tgastine Exp $
# Makefile for generating different output formats of the $(FILE) inspired
# from the Pencil Code one used to build the manual.
#
# Usage:
#  make
#  make $(FILE).pdf
#  make clean
#
# ------------------
FILE             = Gastine
LATEX            = latex -src
DVIPS            = dvips
BIBTEX           = bibtex
PS2PDF           = ps2pdf14 -sPAPERSIZE=a4
MAY_HAVE_CHANGED = 'may have changed. Rerun to get'
MAY_NO_BIBTEX    = 'undefined citations'
# ------------------
.SUFFIXES:            # clear all generic rules and suffixes
.SUFFIXES: .tex .dvi .ps .pdf

.tex.dvi:
	$(LATEX) $*
	if [ `fgrep -c $(MAY_HAVE_CHANGED) $*.log` != '' ]; then \
	    $(LATEX) $*; \
	fi
.dvi.ps:
	$(DVIPS) $* -o $*.ps
.ps.pdf:
	$(PS2PDF) $*.ps $*.pdf
# ------------------

default: $(FILE).ps

all: $(FILE).ps $(FILE).pdf

$(FILE).dvi: $(FILE).tex
	@TEXINPUTS="./texinputs:${TEXINPUTS}"; \
	export TEXINPUTS; \
	echo "TEXINPUTS=$${TEXINPUTS}"; \
	$(LATEX) $(FILE) \
	    && if [ `fgrep -c $(MAY_HAVE_CHANGED) $(FILE).log` != '' ]; then \
	           $(LATEX) $(FILE); \
	       fi \
	    && if [ `fgrep -c $(MAY_NO_BIBTEX) $(FILE).log` != '' ]; then \
	    $(BIBTEX) $(FILE); \
	    $(LATEX) $(FILE); \
	    $(LATEX) $(FILE); \
	       fi

$(FILE).pdf: $(FILE).ps
	$(PS2PDF) $(FILE).ps

$(FILE).ps: $(FILE).dvi
	$(DVIPS) $(FILE) -o $(FILE).ps

bib:
	bibtex $(FILE)

# Clean up
clean:
	rm -f $(FILE).ps* $(FILE).dvi *.aux *.toc *.log *.bbl *.blg *.nav *.snm \
	$(FILE).pdf $(FILE).out $(FILE).tex.backup $(FILE).tex~

# End of file

